Fair and Efficient Gossip in Hyperledger Fabric

Permissioned blockchains are supported by identified but individually untrustworthy nodes, collectively maintaining a replicated ledger whose content is trusted. The Hyperledger Fabric permissioned blockchain system targets high-throughput transaction processing. Fabric uses a set of nodes tasked with the ordering of transactions using consensus. Additional peers endorse and validate transactions, and maintain a copy of the ledger. The ability to quickly disseminate new transaction blocks from ordering nodes to all peers is critical for both performance and consistency. Broadcast is handled by a gossip protocol, using randomized exchanges of blocks between peers. We show that the current implementation of gossip in Fabric leads to heavy tail distributions of block propagation latencies, impacting performance, consistency, and fairness. We contribute a novel design for gossip in Fabric that simultaneously optimizes propagation time, tail latency and bandwidth consumption. Using a 100-node cluster, we show that our enhanced gossip allows the dissemination of blocks to all peers more than 10 times faster than with the original implementation, while decreasing the overall network bandwidth consumption by more than 40%. With a high throughput and concurrent application, this results in 17% to 36% fewer invalidated transactions for different block sizes.

==> implementation.tex <==
%!TEX root = paper.tex

% --------------------

\vspace{-1mm}
\section{Implementation}
\label{section:implementation}

As shown in the previous section, if we associate each block a time-to-live (TTL), we can compute the number of times it needs to be sent during the push phase in order to have all the nodes informed with high probability.
After such a push phase, the entire network receives the block with high probability making the pull phase redundant.

We have therefore disabled the gossip via pull for block messages and attached them a TTL.
In addition, instead of forwarding a block only the first time it is received (infect-on-contagion model), peers forward block messages each time they receive one (infect-on-contagion model).

Because sending these many messages would worsen the number of double receptions, we have replaced some of the push rounds with a push proposal phase in which a new block is advertised to randomly chosen peers which in turn request it if needed.
The TTL is thus composed from two values:
\begin{itemize}
	\item push TTL - the number of rounds a block is pushed
	\item advertise TTL - the number of rounds a block is advertised
\end{itemize}
At first, the block is sent directly in order to maximize the number of peer receiving it while keeping the count of double receptions at a minimum. After this phase, the block will be advertised for the rest of the rounds.

% --------------------

